X-RiSAWOZ: High-Quality End-to-End Multilingual Dialogue Datasets and Few-shot Agents

Task-oriented dialogue research has mainly focused on a few popular languages like English and Chinese, due to the high dataset creation cost for a new language. To reduce the cost, we apply manual editing to automatically translated data. We create a new multilingual benchmark, X-RiSAWOZ, by translating the Chinese RiSAWOZ to 4 languages: English, French, Hindi, Korean; and a code-mixed English-Hindi language. X-RiSAWOZ has more than 18,000 human-verified dialogue utterances for each language, and unlike most multilingual prior work, is an end-to-end dataset for building fully-functioning agents. The many difficulties we encountered in creating X-RiSAWOZ led us to develop a toolset to accelerate the post-editing of a new language dataset after translation. This toolset improves machine translation with a hybrid entity alignment technique that combines neural with dictionary-based methods, along with many automated and semi-automated validation checks. We establish strong baselines for X-RiSAWOZ by training dialogue agents in the zero- and few-shot settings where limited gold data is available in the target language. Our results suggest that our translation and post-editing methodology and toolset can be used to create new high-quality multilingual dialogue agents cost-effectively. Our dataset, code, and toolkit are released open-source.

==> method.tex <==
\section{Automatic Labeling}
\label{method}

So far, we have discussed how we leverage training data gathered for a different language. As the agent is deployed, we will start seeing native data in the target language that reflects real usage. Here we propose an automatic method to turn unannotated data into an effective training data set. 

Our proposal is to train a {\em label error classifier} which accepts a sentence and an annotation generated by a given semantic parser and predicts if the annotation is correct. This classifier is trained with data synthesized to mimic the behavior of a given semantic parser.

We use this classifier to self-train the semantic parser. We use the semantic parser to annotate the new data, and only those input and resulting annotation pairs classified as correct are chosen as training data to further fine-tune the model.



\subsection{A Label Error Classifier}

\begin{table}[!htb]
\fontsize{8}{10}\selectfont
\begin{tabularx}{\linewidth}{l|X}
\hline
      \bf Perturbation              & \bf Dialogue state                                                                                                                                                                                                                                                   \\ \hline
\multirow{1}{*}{\bf None (Gold)}              & ( hotel ) hotel\_type  " business " , pricerange  " cheap "                                                \\ \hline
\multirow{1}{*}{\bf Omit a slot}        & ( hotel ) ( hotel ) hotel\_type  " business "   \\ \hline
\multirow{2}{*}{\bf Wrong slot-value}    & ( hotel ) hotel\_type  " business " , pricerange  " medium "     \\ \hline
\multirow{2}{*}{\bf Hallucinate a slot}  & ( hotel ) hotel\_type  " business " , pricerange  " cheap " , stars " 3 "  \\ \hline
\end{tabularx}
\caption{Perturbation types for DST}
\label{tab:perturb-types}
\end{table}


\begin{table}[!htb]
\newcolumntype{M}{>{\arraybackslash}m{1.5cm}}
\fontsize{8}{10}\selectfont
\begin{tabularx}{\linewidth}{l|X}
\hline
\bf Perturbation      & \bf Dialogue Act  \\ \hline
\multirow{2}{*}{\bf None (Gold)}         & ( attraction ) inform ticket\_price  " 45 yuan "   \\ \hline
\multirow{1}{*}{\bf Omit an act}       & ( attraction )  general \\ \hline
\multirow{3}{*}{\bf Hallucinate an act} & ( attraction ) inform ticket\_price  " 45 yuan " , inform name " Japanese Garden "             \\ \hline
\end{tabularx}
\caption{Perturbation types for DA}
\label{tab:perturb-types-da}
\end{table}

We train a classifier to judge whether the output of the semantic parser is correct given the input. The input to the classifier is the concatenation of the input and output of the semantic parser. The output is a binary value: 0 indicating the output is a correct annotation (positive example) and 1 otherwise (negative example). To train a robust error classifier, we synthesize more negative examples that mimic the kinds of errors the zero-shot model is prone to making. 

During an initial error analysis of the zero-shot model predictions, we noticed that model errors tend to follow certain patterns. 

For DST, we group the errors into three types. For the correct output, the model can omit, hallucinate, or mispredict a slot-value pair. In order to train our classifier, for each domain, we compute the statistics of the most common slots for which each of these error types occurs in. Then, for each slot, we find all possible turns in which we can perturb the gold output to mimic the same error types, shown in Table \ref{tab:perturb-types}. The goal is to generate as many perturbations as possible that mimic the type of error that was made on harder turns, to train a robust error detection classifier.

For DA, a similar process can be applied, except now every turn comes with (act, slot, value) triplets instead of (slot, value) pairs. Our analysis shows errors happen at the act-level, so we create perturbations as shown in Table \ref{tab:perturb-types-da}. 

For DST, we observed training one classifier is not sufficient to achieve high recall. Instead, we train an ensemble of $k$ classifiers $\{g_i : 1\le i \le k\}$, with each independent classifier $g_i$ procured using the same process but different random seeds. An example $x$ is filtered if $\min(1, \sum_i g_i(x)) = 1$. This way, we greatly expand coverage of negative error types.
